RayleighBloch waves above the cut-off

Extensions of Rayleigh-Bloch waves above the cut-off frequency are studied via the discrete spectrum of a transfer operator for a generalised channel containing a single cylinder. Their wavenumbers are shown to become complex-valued and an additional pair of wavenumbers to appear. For small to intermediate radius values, the extended Rayleigh-Bloch waves are shown connect the Neumann and Dirichlet trapped modes, then embed in the continuous spectrum. Rayleigh-Bloch waves vanish as frequency increases but reappear at high frequencies for small and large cylinders. The existence and properties of the Rayleigh-Bloch waves are connected with finite-array resonances.

==> Figs/Fig_Evals.tex <==
\input{./definitions-luke-fig}
\input{../colours-luke}

%\def\figwidth{240pt}

\newlength{\figurewidth}
\newlength{\figwidth}
\newlength{\colsep}
\newlength{\figureheight}
\newlength{\myxunit}
\newlength{\rad}

%\newlength{\pagewidth}
\setlength{\pagewidth}{7.5cm}

\begin{document}

\begin{my}

\centering

%\setlength{\figureheight}{1.2\pagewidth} 
%\setlength{\figurewidth}{\figureheight} 
%\setlength{\colsep}{0.009\figurewidth} 

\setlength{\figurewidth}{0.2\textwidth} 
\setlength{\figureheight}{0.2\textwidth} 
\setlength{\colsep}{0.2\figurewidth} 
\begin{tikzpicture}
\input{evals_k-1.950}
\input{dirspec_k-1.950}
\input{efn_surf_k-1.950_s-5.0}
%
\input{evals_k-1.500}
\input{dirspec_k-1.500}
\input{efn_surf_k-1.500_s-5.0}
%
\input{evals_k-1.119}
\input{dirspec_k-1.119}
\input{efn_surf_k-1.119_s-5.0}
%
\input{evals_k-0.900}
\input{dirspec_k-0.900}
\input{efn_surf_k-0.900_s-5.0}
%
\input{evals_k-0.800}
\input{dirspec_k-0.800}
\input{efn_surf_k-0.800_s-5.0}
\end{tikzpicture}


\end{my}

\end{document}


==> Figs/efn_surf_k-1.950_s-5.0.tex <==
% !TEX root = ../RayBl_cutoff.tex

% This file was created by matlab2tikz.
%
/
\begin{axis}[%
name=2er,
width=0.2\figurewidth,
height=\figureheight,
at={($(2em.east)+(\colsep,0)$)}, %{(0\figurewidth,0.8\figureheight)}, %
anchor=west,
scale only axis,
%point meta min=-6.47979628743317,
%point meta max=6.47979628743317,
colormap/jet,
xmin=-0.5,
xmax=0.5,
%xtick={-0.5,0.5},
%xlabel style={font=\color{white!15!black}},
xticklabels={\none},
%xlabel={$x$},
ymin=-2.5,
ymax=2.5,
yticklabels={\none},
axis line style={draw=none},
%ticks=none,
%title style={font=\bfseries},
%title={}, %{$k = 0.8000\pi$; $q = 0.8282\pi + 0.0000$i},
%axis x line*=bottom,
%axis y line*=left,
%xmajorgrids,
%ymajorgrids,
legend style={legend cell align=left, align=left, draw=white!15!black},
%colorbar
]

\addplot[area legend, draw=none, table/row sep=crcr, patch, shader=interp, patch table={%
55	71	32\\
76	36	75\\
3	75	36\\
35	75	3\\
58	89	56\\
56	30	58\\
99	71	88\\
59	58	30\\
86	85	113\\
134	112	64\\
64	12	44\\
26	59	30\\
57	82	115\\
57	26	23\\
59	26	57\\
89	58	116\\
58	59	116\\
61	62	97\\
115	82	117\\
84	90	143\\
144	113	85\\
86	113	114\\
29	57	23\\
82	57	29\\
120	117	87\\
87	117	82\\
136	62	96\\
97	62	136\\
125	75	102\\
122	100	72\\
0	32	72\\
72	99	122\\
72	32	71\\
71	99	72\\
76	75	103\\
103	75	125\\
44	11	65\\
65	64	44\\
59	57	118\\
118	116	59\\
98	61	137\\
137	61	97\\
14	62	47\\
62	61	47\\
92	144	85\\
92	84	143\\
85	84	92\\
86	114	60\\
60	28	86\\
24	28	60\\
21	84	52\\
52	84	85\\
31	85	86\\
86	28	31\\
82	29	27\\
27	87	82\\
46	62	14\\
12	64	45\\
81	141	91\\
74	75	35\\
74	102	75\\
124	102	74\\
35	2	74\\
101	124	74\\
74	2	34\\
0	72	33\\
34	1	73\\
73	123	101\\
101	74	73\\
73	74	34\\
100	123	73\\
1	33	73\\
73	72	100\\
73	33	72\\
126	104	76\\
76	103	126\\
70	129	107\\
66	10	42\\
43	65	11\\
43	10	66\\
66	65	43\\
121	57	115\\
121	118	57\\
19	81	53\\
54	84	21\\
91	142	83\\
83	20	53\\
83	54	20\\
83	81	91\\
53	81	83\\
83	142	90\\
90	84	83\\
84	54	83\\
15	61	48\\
15	47	61\\
50	17	79\\
79	139	95\\
94	139	79\\
119	60	114\\
120	87	119\\
87	60	119\\
22	52	85\\
85	31	22\\
87	27	25\\
24	60	25\\
25	60	87\\
63	64	112\\
63	45	64\\
112	135	63\\
13	45	63\\
63	135	96\\
63	46	13\\
96	62	63\\
62	46	63\\
141	81	93\\
4	36	76\\
76	37	4\\
104	127	77\\
5	37	77\\
77	127	105\\
77	38	5\\
76	104	77\\
77	37	76\\
7	70	40\\
68	8	40\\
107	130	68\\
68	70	107\\
40	70	68\\
105	128	69\\
6	38	69\\
69	77	105\\
38	77	69\\
109	132	66\\
110	133	65\\
66	132	110\\
110	65	66\\
134	64	111\\
64	65	111\\
65	133	111\\
49	79	17\\
140	93	80\\
95	140	80\\
80	93	81\\
80	18	50\\
80	79	95\\
50	79	80\\
108	68	130\\
8	68	41\\
6	69	39\\
39	69	70\\
70	7	39\\
106	69	128\\
70	69	106\\
129	70	106\\
78	49	16\\
78	138	94\\
94	79	78\\
79	49	78\\
78	16	48\\
98	138	78\\
78	61	98\\
48	61	78\\
18	80	51\\
51	80	81\\
81	19	51\\
68	108	67\\
67	41	68\\
67	108	131\\
9	41	67\\
131	109	67\\
67	42	9\\
66	42	67\\
67	109	66\\
}]
table[row sep=crcr, point meta=\thisrow{c}] {%
x	y	c\\
-0.700000000121094	-2.32679491905944	-0.00629100133470405\\
-0.700000000121094	-2.15358983784463	-0.00250354810483148\\
-0.700000000121094	-1.98038475546625	-0.0053437965721956\\
-0.700000000121094	-1.80717966920398	-0.0138525816734184\\
-0.700000000121094	-1.63397457065445	-0.0215345510075965\\
-0.700000000121094	-1.4607694351255	-0.0233028788620184\\
-0.700000000121094	-1.28756419371258	-0.0207665991176965\\
-0.700000000121094	-1.11435866388318	-0.0205131605383761\\
-0.700000000121094	-0.941152386797045	-0.0278686573681327\\
-0.700000000121094	-0.767944268581065	-0.0414407256021828\\
-0.700000000121094	-0.594731838196743	-0.0546325226519092\\
-0.700000000121094	-0.421509813444829	-0.0629468239873332\\
-0.700000000121094	-0.248267530352638	-0.0665617249608716\\
-0.700000000121094	-0.0749847081094265	-0.0635020998010173\\
-0.700000000121094	0.0983748886706041	-0.0641932034563451\\
-0.700000000121094	0.271871958148578	-0.0663236815807559\\
-0.700000000121094	0.445601776462654	-0.0621562346763691\\
-0.700000000121094	0.619704561434028	-0.0529600708355265\\
-0.700000000121093	0.794373534320031	-0.0392069111340507\\
-0.700000000121091	0.969856118179784	-0.0261185308853304\\
-0.700000000121085	1.14644256146302	-0.0200459380715598\\
-0.700000000121071	1.32444108337789	-0.0213722594188069\\
-0.700000000120364	1.50578689973314	-0.0234701517861691\\
-0.70000000011879	2.19456095597396	-0.00290507244160669\\
-0.70000000011132	1.79654077967193	-0.0144180284633061\\
-0.70000000011115	1.88839225956867	-0.00952306447675877\\
-0.700000000100456	2.28871337559458	-0.00508201745367422\\
-0.700000000096762	1.98950384581519	-0.00501258504242304\\
-0.700000000095167	1.69753640292769	-0.0192171091542053\\
-0.700000000094478	2.09584690704003	-0.00261837729481729\\
-0.70000000009456	2.39363253791533	-0.00850574997574828\\
-0.700000000093801	1.59587380246177	-0.0225145915868686\\
-0.700000000037599	-2.41339745952568	-0.00912556106270001\\
-0.700000000037599	-2.24019237852158	-0.00377239828729189\\
-0.700000000037599	-2.06698729689904	-0.00298896914030337\\
-0.700000000037599	-1.8937822131349	-0.00924636998302\\
-0.700000000037599	-1.72057712242571	-0.0182032321583452\\
-0.700000000037599	-1.54737201030429	-0.0232635663439975\\
-0.700000000037599	-1.3741668353678	-0.0222106352733157\\
-0.700000000037598	-1.20096148510128	-0.0198693123140658\\
-0.700000000037597	-1.02775566926161	-0.0232060154563807\\
-0.700000000037595	-0.854548677479934	-0.0342042304021242\\
-0.700000000037589	-0.681338861310351	-0.0484637334588158\\
-0.700000000037575	-0.508122597773204	-0.0595726571119779\\
-0.700000000037546	-0.334892357637673	-0.0651871423813442\\
-0.700000000037487	-0.16163337859185	-0.0659519848850234\\
-0.700000000037373	0.0116815742044803	-0.0623553613257348\\
-0.700000000037168	0.185099664077486	-0.0663685198866903\\
-0.700000000036816	0.35869745405548	-0.0646425451211975\\
-0.700000000036245	0.532591471324878	-0.0583299093638377\\
-0.700000000035371	0.706947992605234	-0.0464596545185174\\
-0.700000000034101	0.881988582962275	-0.03204893795478\\
-0.700000000033531	1.41408171454796	-0.0228054822046142\\
-0.70000000003236	1.05798594595702	-0.0220316725594031\\
-0.700000000030109	1.23524585520405	-0.020092156091181\\
-0.7	-2.5	-0.0112916499973502\\
-0.7	2.5	-0.0112916549434608\\
-0.600060216045899	2.18400312733838	-0.00281715065101816\\
-0.600049441998156	2.45940306145265	-0.0107012673991805\\
-0.60002973941679	2.32176697514369	-0.00630245287914414\\
-0.600007725009206	1.77428878076498	-0.014811300614424\\
-0.600000001514186	0.271844901783914	-0.0398613478106944\\
-0.600000001490492	0.0983593755825481	-0.0345605902599701\\
-0.600000000648419	-0.0749930524100742	-0.0340221855655462\\
-0.600000000221625	-0.248271756053237	-0.0391814187544725\\
-0.600000000067343	-0.421511834585219	-0.0425526341408217\\
-0.600000000019051	-0.594732753453041	-0.0400126901207463\\
-0.600000000005086	-0.76794466164736	-0.0310033718110311\\
-0.600000000001281	-0.941152547056804	-0.0205770024082134\\
-0.600000000000067	-1.28756421656046	-0.0172785981042696\\
-0.600000000000303	-1.11435872595504	-0.0154388699212159\\
-0.6	-2.49999999986975	-0.0116234204716683\\
-0.6	-2.32679491907802	-0.00646993427599003\\
-0.6	-2.15358983791694	-0.0025130734397857\\
-0.6	-1.98038475571952	-0.00512604206070063\\
-0.6	-1.80717967004552	-0.0131788290971483\\
-0.600000000000003	-1.63397457331417	-0.0202027912720823\\
-0.600000000000014	-1.46076944312005	-0.0210695895154571\\
-0.599999991783631	0.445557668330762	-0.0426247900127902\\
-0.599999935479976	0.619637621108763	-0.0390522313392746\\
-0.599999717808814	0.794279583759996	-0.0293261426621421\\
-0.599999035138153	0.969735907206737	-0.0192326885484273\\
-0.59999819098712	2.04649740847848	-0.00326076767536181\\
-0.599997152549104	1.14630677922418	-0.0153235062992676\\
-0.599992405353538	1.3243166725119	-0.0181702748240822\\
-0.599978477090023	1.50007788344362	-0.0214528771534506\\
-0.599970269065746	1.63719071003995	-0.0201197896331458\\
-0.599967917953738	1.91030715706806	-0.00803329058869343\\
-0.5	-2.5	-0.00957851256791948\\
-0.5	2.5	-0.00957851264808441\\
-0.499999999969858	1.23527956625295	-0.00500075912757362\\
-0.499999999967628	1.05799674304258	-0.00207791588093633\\
-0.499999999966373	1.41417601547651	-0.0114943939246691\\
-0.499999999965895	0.881991526086673	-0.00577025980313593\\
-0.499999999963754	0.532591522277105	-0.0124334956053937\\
-0.499999999964628	0.706948597017265	-0.0116538634729839\\
-0.499999999962627	0.011681566425207	0.0110484258244554\\
-0.499999999962832	0.185099644911972	0.00539964771976326\\
-0.499999999963184	0.358697426147969	-0.00524720502874298\\
-0.499999999962401	-2.41339745952568	-0.00705558076145043\\
-0.499999999962401	-2.24019237852158	-0.00100169090345633\\
-0.499999999962401	-2.06698729689904	0.000699295749214654\\
-0.499999999962401	-1.8937822131349	-0.0043072808579582\\
-0.499999999962401	-1.72057712242571	-0.0115229957154734\\
-0.499999999962401	-1.54737201030432	-0.0141767742594854\\
-0.499999999962401	-1.37416683536795	-0.0101178415890085\\
-0.499999999962401	-1.20096148510201	-0.00396116877201215\\
-0.499999999962403	-1.02775566926492	-0.00227653403003111\\
-0.499999999962405	-0.854548677494083	-0.00673726539428308\\
-0.499999999962411	-0.681338861367236	-0.0122345661008229\\
-0.499999999962425	-0.50812259798907	-0.0118761107478629\\
-0.499999999962454	-0.334892358411163	-0.00381800803602911\\
-0.499999999962513	-0.161633381178732	0.00664227563933305\\
-0.499999999906024	1.59611420576089	-0.0141525254036546\\
-0.499999999904735	1.69790647097738	-0.0122464784353833\\
-0.499999999905666	2.09640722552543	0.000910928309404567\\
-0.499999999905743	2.39389140632676	-0.00636452761711293\\
-0.499999999903137	1.99003521516067	-0.000828376470438445\\
-0.499999999899003	2.28929781970588	-0.00254140795290179\\
-0.49999999988926	1.79715441491457	-0.00853090330731815\\
-0.4999999998881	1.88906300850426	-0.00450695629314174\\
-0.499999999881897	2.19528211529381	7.56652939574423e-05\\
-0.499999999878906	-2.32679491905944	-0.00387999096944897\\
-0.499999999878906	-2.15358983784463	0.00070853196660633\\
-0.499999999878906	-1.98038475546625	-0.00111022240543252\\
-0.499999999878906	-1.80717966920398	-0.00809746466758633\\
-0.499999999878906	-1.63397457065447	-0.0137249277730702\\
-0.499999999878906	-1.46076943512559	-0.0128283378126418\\
-0.499999999878906	-1.28756419371302	-0.00684761368496785\\
-0.499999999878906	-1.11435866388526	-0.00228101021858002\\
-0.499999999878906	-0.941152386806261	-0.00393015835912198\\
-0.499999999878906	-0.767944268619261	-0.00983572717588876\\
-0.499999999878906	-0.594731838345899	-0.01307931664133\\
-0.499999999878906	-0.421509813995169	-0.00862240686875389\\
-0.499999999878906	-0.248267532263179	0.00164207455069744\\
-0.499999999878906	-0.0749847142129475	0.0100593307371032\\
-0.499999999878906	0.098374871748858	0.0093493135802554\\
-0.499999999878906	0.271871923370587	0.000150899602672695\\
-0.499999999878906	0.445601760019517	-0.00971304293614865\\
-0.499999999878906	0.619704854266866	-0.013032664163792\\
-0.499999999878905	0.794375409933814	-0.00891886883194678\\
-0.499999999878904	0.969863879294993	-0.00322022071800631\\
-0.499999999878898	1.14646867299888	-0.00272375056005326\\
-0.499999999878884	1.32451818471685	-0.00825115724256033\\
-0.499999999879558	1.50599392551501	-0.0137407537028446\\
};
%\addlegendentry{data1}


\addplot[area legend, draw=none, table/row sep=crcr, patch, shader=interp, patch table={%
99	67	88\\
55	67	32\\
68	99	123\\
0	32	68\\
67	99	68\\
68	32	67\\
34	69	70\\
120	84	119\\
66	16	48\\
22	59	31\\
122	59	92\\
31	59	58\\
58	28	31\\
84	28	58\\
73	5	37\\
86	89	56\\
100	68	123\\
69	68	100\\
100	124	69\\
0	68	33\\
33	68	69\\
70	35	2\\
2	34	70\\
82	81	96\\
59	22	52\\
25	28	84\\
113	59	122\\
113	58	59\\
30	86	56\\
85	86	30\\
116	86	85\\
85	118	116\\
89	86	116\\
121	118	87\\
87	118	85\\
76	8	40\\
37	4	72\\
72	73	37\\
104	73	72\\
69	34	1\\
1	33	69\\
82	47	14\\
83	47	82\\
83	66	48\\
98	66	83\\
45	81	13\\
98	83	138\\
58	113	114\\
114	119	84\\
84	58	114\\
110	78	133\\
133	78	109\\
109	78	77\\
77	132	109\\
10	78	43\\
134	111	79\\
44	11	79\\
79	110	134\\
11	43	79\\
78	110	79\\
79	43	78\\
85	30	26\\
26	87	85\\
23	87	26\\
121	87	115\\
77	9	41\\
41	76	77\\
8	76	41\\
42	78	10\\
77	78	42\\
42	9	77\\
108	132	77\\
77	76	108\\
104	72	127\\
36	72	4\\
101	125	70\\
70	69	101\\
69	124	101\\
70	125	102\\
82	14	46\\
13	81	46\\
46	81	82\\
15	83	48\\
47	83	15\\
82	96	137\\
139	66	98\\
139	94	66\\
81	45	80\\
80	112	81\\
135	112	80\\
80	45	12\\
80	111	135\\
80	12	44\\
44	79	80\\
80	79	111\\
144	92	60\\
60	52	21\\
60	92	59\\
59	52	60\\
128	73	104\\
128	105	73\\
40	7	75\\
75	130	107\\
107	76	75\\
75	76	40\\
29	87	23\\
57	27	24\\
120	117	57\\
57	84	120\\
24	25	57\\
57	25	84\\
5	73	38\\
131	76	107\\
131	108	76\\
71	36	3\\
71	3	35\\
71	102	126\\
72	36	71\\
71	35	70\\
70	102	71\\
136	96	81\\
81	112	136\\
97	83	82\\
82	137	97\\
97	138	83\\
144	60	90\\
63	19	51\\
66	94	65\\
65	94	140\\
130	75	106\\
39	75	7\\
62	115	87\\
87	29	62\\
62	29	27\\
117	115	62\\
62	57	117\\
27	57	62\\
103	71	126\\
72	71	103\\
103	127	72\\
54	60	21\\
91	63	142\\
19	63	53\\
142	63	93\\
16	66	49\\
66	65	49\\
95	65	140\\
129	106	74\\
74	39	6\\
74	105	129\\
6	38	74\\
74	106	75\\
75	39	74\\
73	105	74\\
74	38	73\\
63	91	61\\
61	53	63\\
61	91	143\\
20	53	61\\
143	90	61\\
61	54	20\\
61	90	60\\
60	54	61\\
17	65	50\\
17	49	65\\
50	65	64\\
65	95	64\\
64	95	141\\
64	18	50\\
141	93	64\\
51	18	64\\
64	63	51\\
64	93	63\\
}]
table[row sep=crcr, point meta=\thisrow{c}] {%
x	y	c\\
0.499999999878906	-2.32679491905944	-0.00362723308223919\\
0.499999999878906	-2.15358983784463	0.000484504684689802\\
0.499999999878906	-1.98038475546625	-0.00187719250735743\\
0.499999999878906	-1.80717966920398	-0.00897339835782723\\
0.499999999878906	-1.63397457065447	-0.0142276460135726\\
0.499999999878906	-1.46076943512559	-0.0129287888261181\\
0.499999999878906	-1.28756419371302	-0.00700678313178804\\
0.499999999878906	-1.11435866388526	-0.00298386009134534\\
0.499999999878906	-0.941152386806261	-0.00519244992337825\\
0.499999999878906	-0.767944268619261	-0.0111870695676019\\
0.499999999878906	-0.594731838345899	-0.0140365962977426\\
0.499999999878906	-0.421509813995169	-0.00916004896083891\\
0.499999999878906	-0.248267532263179	0.00113427197126671\\
0.499999999878906	-0.0749847142129475	0.00933233926563014\\
0.499999999878906	0.098374871748858	0.00864671376935599\\
0.499999999878906	0.271871923370587	-0.000336279803929576\\
0.499999999878906	0.445601760019517	-0.0102907466487587\\
0.499999999878906	0.619704854266866	-0.014061738554667\\
0.499999999878905	0.794375409933815	-0.0102944541266441\\
0.499999999878904	0.969863879294994	-0.00441329559198558\\
0.499999999878898	1.14646867299889	-0.00330672916787521\\
0.499999999878884	1.32451818471685	-0.00834864675206094\\
0.499999999879558	1.50599392551501	-0.0139163256896152\\
0.499999999881897	2.1952821152938	-5.3567013468701e-06\\
0.4999999998881	1.88906300850423	-0.00540272734825831\\
0.49999999988926	1.79715441491454	-0.00939584361696482\\
0.499999999899003	2.28929781970588	-0.00235806564988268\\
0.499999999903137	1.99003521516067	-0.00157323828145523\\
0.499999999904735	1.69790647097738	-0.0129215483523586\\
0.499999999905666	2.09640722552543	0.000485769405053311\\
0.499999999905743	2.39389140632676	-0.00605345097874649\\
0.499999999906024	1.59611420576089	-0.0145490943123278\\
0.499999999962401	-2.41339745952568	-0.00674433822218222\\
0.499999999962401	-2.24019237852158	-0.000943047464287734\\
0.499999999962401	-2.06698729689904	0.000174960354280317\\
0.499999999962401	-1.8937822131349	-0.00520023867283777\\
0.499999999962401	-1.72057712242571	-0.0122523333101539\\
0.499999999962401	-1.54737201030432	-0.0144449462827533\\
0.499999999962401	-1.37416683536795	-0.0101742001186971\\
0.499999999962401	-1.20096148510201	-0.0043532837600664\\
0.499999999962403	-1.02775566926492	-0.00329435416421454\\
0.499999999962405	-0.854548677494083	-0.00811787362613547\\
0.499999999962411	-0.681338861367236	-0.0134273611681353\\
0.499999999962425	-0.50812259798907	-0.0125920660562145\\
0.499999999962454	-0.334892358411163	-0.00428491487365813\\
0.499999999962513	-0.161633381178732	0.00602333642429859\\
0.499999999962627	0.011681566425207	0.0102858420883293\\
0.499999999962832	0.185099644911972	0.00481387079654286\\
0.499999999963184	0.358697426147969	-0.00572175598266523\\
0.499999999963754	0.532591522277105	-0.0132139490877472\\
0.499999999964628	0.706948597017265	-0.0129044351927863\\
0.499999999965895	0.881991526086674	-0.00712912176087043\\
0.499999999966373	1.41417601547651	-0.0115533664598488\\
0.499999999967628	1.05799674304258	-0.00299015550475779\\
0.499999999969858	1.23527956625295	-0.00528767991472703\\
0.5	-2.5	-0.00935465407728337\\
0.5	2.5	-0.00935465416839459\\
0.599967917953738	1.91030715706811	0.00171807026547601\\
0.599970269065746	1.63719071003999	-0.00574140064461537\\
0.599978477090022	1.50007788344364	-0.00396203019317371\\
0.599992405353537	1.3243166725119	0.0036090356544571\\
0.599997152549104	1.14630677922418	0.0111841455824139\\
0.59999819098712	2.04649740847852	0.00521988101294199\\
0.599999035138153	0.969735907206738	0.013157962601286\\
0.599999717808814	0.794279583759996	0.0110804438770542\\
0.599999935479976	0.619637621108763	0.0119613010106962\\
0.599999991783631	0.445557668330763	0.0211758805979863\\
0.6	-2.49999999986975	-0.00599734307377525\\
0.6	-2.32679491907802	0.000416852403817734\\
0.6	-2.15358983791694	0.00530842259294904\\
0.6	-1.98038475571952	0.0038929749669439\\
0.600000000000001	-1.80717967004552	-0.0019996769447759\\
0.600000000000003	-1.63397457331417	-0.00575131086733017\\
0.600000000000014	-1.46076944312005	-0.00264034656711915\\
0.600000000000067	-1.28756421656046	0.00543079767525394\\
0.600000000000303	-1.11435872595504	0.0120172921808741\\
0.600000000001281	-0.941152547056804	0.0129454922315548\\
0.600000000005086	-0.76794466164736	0.0108356278901555\\
0.600000000019051	-0.594732753453041	0.012722757490925\\
0.600000000067343	-0.421511834585219	0.0230880000318815\\
0.600000000221625	-0.248271756053237	0.0385929326812661\\
0.600000000648419	-0.0749930524100743	0.0492903270767328\\
0.600000001490492	0.0983593755825481	0.0484650831189959\\
0.600000001514186	0.271844901783914	0.0365182476879166\\
0.600007725009207	1.77428878076504	-0.00309119782626534\\
0.60002973941679	2.32176697514371	0.000615809368792694\\
0.600049441998157	2.45940306145267	-0.00473650022428242\\
0.6000602160459	2.18400312733841	0.00484569076574859\\
0.7	-2.5	-0.0022098689683746\\
0.7	2.5	-0.00220986896961479\\
0.700000000030109	1.23524585520405	0.019375542252043\\
0.70000000003236	1.05798594595702	0.026242074955608\\
0.700000000033531	1.41408171454796	0.00917617490144799\\
0.700000000034101	0.881988582962276	0.0274953581921763\\
0.700000000036245	0.532591471324878	0.0356033977435802\\
0.700000000035371	0.706947992605234	0.0282462671746348\\
0.700000000037373	0.0116815742044803	0.0760691279461526\\
0.700000000037168	0.185099664077486	0.0694846197412916\\
0.700000000036816	0.35869745405548	0.051593688046425\\
0.700000000037599	-2.41339745952568	0.00106438149862277\\
0.700000000037599	-2.24019237852158	0.00824520878134925\\
0.700000000037599	-2.06698729689904	0.0109758867431062\\
0.700000000037599	-1.8937822131349	0.00756814794314908\\
0.700000000037599	-1.72057712242571	0.00294872822356178\\
0.700000000037599	-1.54737201030429	0.0037188365547681\\
0.700000000037599	-1.3741668353678	0.0113895398326557\\
0.700000000037598	-1.20096148510128	0.0211206553804957\\
0.700000000037597	-1.02775566926161	0.0268023807163575\\
0.700000000037595	-0.854548677479934	0.0274563341069789\\
0.700000000037589	-0.681338861310351	0.0287590207892438\\
0.700000000037575	-0.508122597773204	0.0373996739215972\\
0.700000000037546	-0.334892357637673	0.0542189888551977\\
0.700000000037487	-0.16163337859185	0.0711952811297166\\
0.700000000093801	1.59587380246177	0.00274190670062849\\
0.700000000095167	1.69753640292768	0.00263286089302375\\
0.700000000094478	2.09584690704002	0.0109989537544352\\
0.70000000009456	2.39363253791533	0.00191811624714622\\
0.700000000096762	1.98950384581518	0.0100247053427088\\
0.700000000100456	2.28871337559457	0.00644577616043737\\
0.70000000011132	1.7965407796719	0.00465857878011336\\
0.70000000011115	1.88839225956863	0.0074063975650528\\
0.70000000011879	2.19456095597394	0.00959628179817795\\
0.700000000120364	1.50578689973313	0.00501809293368171\\
0.700000000121094	-2.32679491905944	0.00485518028233447\\
0.700000000121094	-2.15358983784463	0.0104513105686761\\
0.700000000121094	-1.98038475546625	0.00983951942319602\\
0.700000000121094	-1.80717966920398	0.00495743381298539\\
0.700000000121094	-1.63397457065445	0.0023970464755817\\
0.700000000121094	-1.4607694351255	0.00686191874716921\\
0.700000000121094	-1.28756419371258	0.0164599547708299\\
0.700000000121094	-1.11435866388318	0.024693580645177\\
0.700000000121094	-0.941152386797045	0.0275022772792361\\
0.700000000121094	-0.767944268581065	0.0275806827163732\\
0.700000000121094	-0.594731838196743	0.0318802553816695\\
0.700000000121094	-0.421509813444829	0.045043726346674\\
0.700000000121094	-0.248267530352638	0.0636916844570936\\
0.700000000121094	-0.0749847081094266	0.0751641143176145\\
0.700000000121094	0.098374888670604	0.0744411657285529\\
0.700000000121094	0.271871958148578	0.0612009770191716\\
0.700000000121094	0.445601776462654	0.0427346291334086\\
0.700000000121094	0.619704561434028	0.0307391664885352\\
0.700000000121093	0.794373534320032	0.0274721964002646\\
0.700000000121091	0.969856118179785	0.0273961978159372\\
0.700000000121085	1.14644256146303	0.0235267789690601\\
0.700000000121071	1.32444108337789	0.0142992338586053\\
};
%\addlegendentry{data2}


\addplot[area legend, draw=none, table/row sep=crcr, patch, shader=interp, patch table={%
142	85	111\\
85	54	111\\
104	43	67\\
43	10	67\\
143	196	123\\
35	28	80\\
308	279	297\\
114	85	142\\
142	171	114\\
20	54	85\\
45	71	14\\
14	71	50\\
98	71	45\\
137	71	98\\
328	344	287\\
109	71	137\\
50	71	109\\
165	109	137\\
273	221	247\\
27	23	88\\
82	88	23\\
169	123	196\\
172	196	143\\
35	80	90\\
80	138	90\\
514	568	532\\
362	388	416\\
445	473	416\\
416	388	445\\
199	171	142\\
199	225	171\\
85	114	73\\
56	20	73\\
73	20	85\\
266	290	321\\
137	98	152\\
152	98	121\\
121	179	152\\
148	179	121\\
176	148	118\\
76	98	45\\
121	98	76\\
207	152	179\\
408	382	439\\
193	247	221\\
50	109	69\\
587	530	534\\
533	530	587\\
68	43	104\\
72	37	15\\
72	94	37\\
143	123	86\\
86	88	143\\
27	88	86\\
74	91	115\\
174	149	115\\
228	174	202\\
33	82	23\\
113	169	170\\
123	169	113\\
226	172	173\\
122	149	173\\
143	88	141\\
141	172	143\\
141	82	122\\
88	82	141\\
122	173	141\\
141	173	172\\
196	172	227\\
227	226	278\\
227	172	226\\
274	224	250\\
252	224	274\\
197	224	252\\
283	252	274\\
276	252	283\\
504	567	566\\
501	567	504\\
501	504	464\\
464	504	474\\
203	231	176\\
471	495	441\\
441	495	469\\
439	382	411\\
411	469	439\\
384	441	411\\
411	441	469\\
150	177	116\\
116	90	150\\
150	90	138\\
150	138	197\\
168	224	197\\
197	138	168\\
297	310	334\\
388	362	334\\
334	308	297\\
334	362	308\\
388	334	364\\
364	334	310\\
502	514	473\\
473	445	502\\
568	514	502\\
502	533	568\\
225	199	253\\
297	279	253\\
279	225	253\\
263	324	295\\
294	324	263\\
294	266	321\\
236	294	263\\
266	294	236\\
205	148	176\\
179	148	205\\
176	231	205\\
231	257	205\\
116	177	146\\
177	203	146\\
176	118	146\\
146	203	176\\
78	118	93\\
93	118	148\\
93	36	78\\
76	36	93\\
93	148	121\\
121	76	93\\
189	207	243\\
189	165	137\\
137	152	189\\
152	207	189\\
466	408	439\\
435	408	466\\
439	469	494\\
494	466	439\\
511	466	494\\
435	466	489\\
489	466	511\\
382	408	354\\
380	408	435\\
380	354	408\\
380	344	328\\
328	354	380\\
273	247	288\\
321	290	347\\
539	518	577\\
164	193	221\\
109	165	136\\
136	69	109\\
165	193	136\\
193	164	136\\
484	534	530\\
104	67	131\\
100	131	67\\
66	100	42\\
42	67	10\\
42	100	67\\
280	281	307\\
278	226	280\\
280	307	278\\
46	13	70\\
46	72	15\\
70	13	44\\
43	68	11\\
68	44	11\\
117	94	147\\
18	37	75\\
37	94	75\\
75	94	117\\
117	91	75\\
75	34	18\\
91	34	75\\
102	46	70\\
72	46	102\\
74	26	22\\
22	91	74\\
22	34	91\\
89	149	122\\
122	82	89\\
74	115	89\\
89	115	149\\
89	26	74\\
82	33	89\\
89	33	26\\
281	280	229\\
226	173	229\\
229	280	226\\
145	91	117\\
145	115	91\\
174	115	145\\
145	202	174\\
175	204	230\\
230	202	175\\
175	147	204\\
117	147	175\\
175	145	117\\
202	145	175\\
365	396	339\\
365	336	392\\
433	396	457\\
339	396	375\\
375	396	433\\
433	457	492\\
83	86	123\\
123	113	83\\
170	200	139\\
139	113	170\\
84	87	24\\
84	83	113\\
113	139	84\\
84	139	87\\
206	252	276\\
197	252	206\\
206	150	197\\
177	150	206\\
274	250	282\\
313	282	337\\
313	283	274\\
274	282	313\\
561	508	570\\
507	508	561\\
243	207	259\\
328	287	259\\
259	287	243\\
285	257	231\\
233	207	179\\
179	205	233\\
233	205	257\\
233	259	207\\
471	437	497\\
355	284	311\\
276	283	311\\
311	284	276\\
384	355	410\\
410	437	471\\
471	441	410\\
410	441	384\\
495	557	555\\
510	495	471\\
510	557	495\\
471	497	510\\
558	557	510\\
510	497	558\\
79	80	28\\
28	17	79\\
116	146	92\\
92	118	78\\
92	146	118\\
77	90	116\\
116	92	77\\
77	92	30\\
338	364	310\\
420	445	388\\
388	364	420\\
530	533	476\\
533	502	476\\
476	502	445\\
445	420	476\\
371	338	319\\
159	127	185\\
16	76	45\\
16	36	76\\
78	36	25\\
247	193	220\\
220	189	243\\
220	193	165\\
165	189	220\\
509	494	469\\
469	495	509\\
509	555	563\\
495	555	509\\
551	509	563\\
494	509	551\\
551	571	511\\
511	494	551\\
511	571	542\\
542	489	511\\
435	489	450\\
272	288	247\\
272	220	243\\
247	220	272\\
243	287	272\\
340	288	315\\
344	367	315\\
315	367	340\\
315	287	344\\
315	272	287\\
288	272	315\\
245	221	273\\
273	289	245\\
397	366	423\\
397	425	370\\
340	367	394\\
394	366	340\\
367	422	394\\
423	366	394\\
342	397	370\\
366	397	342\\
321	347	373\\
535	577	518\\
63	49	9\\
9	48	63\\
50	69	12\\
69	48	12\\
63	48	108\\
108	48	69\\
69	136	108\\
108	136	164\\
467	484	427\\
586	534	529\\
534	484	529\\
484	467	529\\
529	467	486\\
529	537	586\\
486	537	529\\
151	183	126\\
61	47	110\\
151	126	96\\
62	5	38\\
153	187	208\\
41	66	8\\
66	42	8\\
560	567	501\\
204	147	178\\
153	208	178\\
234	204	178\\
178	208	234\\
94	72	119\\
119	147	94\\
119	102	153\\
72	102	119\\
153	178	119\\
119	178	147\\
201	173	149\\
201	229	173\\
201	149	174\\
201	174	228\\
281	229	254\\
254	201	228\\
229	201	254\\
291	336	312\\
339	292	312\\
312	365	339\\
336	365	312\\
195	251	222\\
248	191	222\\
275	292	248\\
248	222	275\\
275	222	251\\
275	251	291\\
291	312	275\\
275	312	292\\
248	292	264\\
421	457	396\\
421	365	392\\
396	365	421\\
421	477	457\\
406	375	433\\
350	375	406\\
27	86	19\\
86	83	19\\
144	139	200\\
87	139	144\\
144	79	87\\
24	87	31\\
87	79	31\\
31	79	17\\
443	419	389\\
507	497	449\\
449	497	437\\
449	437	390\\
390	419	449\\
278	307	309\\
474	448	417\\
475	508	507\\
507	449	475\\
475	449	419\\
475	419	443\\
443	508	475\\
507	561	552\\
558	497	552\\
552	497	507\\
443	448	500\\
500	508	443\\
328	259	286\\
286	354	328\\
286	233	257\\
259	233	286\\
356	411	382\\
384	411	356\\
276	284	232\\
232	206	276\\
232	203	177\\
177	206	232\\
256	285	231\\
256	232	284\\
231	203	256\\
203	232	256\\
355	311	381\\
381	410	355\\
390	437	381\\
437	410	381\\
283	313	335\\
335	311	283\\
390	381	335\\
335	381	311\\
29	77	30\\
35	90	29\\
90	77	29\\
371	427	393\\
393	420	364\\
393	338	371\\
364	338	393\\
324	376	352\\
352	295	324\\
352	319	295\\
371	319	352\\
211	236	263\\
263	295	235\\
235	211	263\\
167	199	142\\
142	111	167\\
111	133	167\\
194	167	133\\
194	160	216\\
133	160	194\\
277	310	297\\
297	253	277\\
106	49	63\\
49	106	60\\
60	106	127\\
53	0	58\\
58	0	52\\
52	101	58\\
214	159	185\\
266	236	214\\
59	52	3\\
101	52	59\\
30	92	32\\
32	92	78\\
78	25	32\\
344	380	398\\
398	367	344\\
398	380	435\\
435	450	398\\
398	422	367\\
450	422	398\\
423	394	451\\
451	394	422\\
478	422	450\\
478	535	518\\
518	451	478\\
478	451	422\\
290	266	240\\
266	214	240\\
240	214	185\\
455	397	423\\
425	397	455\\
370	347	318\\
318	342	370\\
318	347	290\\
289	342	318\\
314	342	289\\
314	288	340\\
340	366	314\\
366	342	314\\
273	288	314\\
314	289	273\\
536	527	584\\
423	451	479\\
479	451	518\\
479	455	423\\
524	455	479\\
479	518	539\\
539	524	479\\
583	524	539\\
584	527	540\\
524	583	540\\
402	347	370\\
402	373	347\\
370	425	402\\
321	373	351\\
351	294	321\\
324	294	351\\
351	376	324\\
49	60	2\\
371	352	407\\
407	352	376\\
407	427	371\\
407	467	427\\
81	140	110\\
81	47	55\\
110	47	81\\
110	140	166\\
166	222	191\\
166	140	195\\
195	222	166\\
4	61	38\\
47	61	4\\
5	62	39\\
39	62	96\\
38	61	95\\
95	62	38\\
154	181	125\\
125	181	151\\
125	95	154\\
62	95	125\\
151	96	125\\
96	62	125\\
383	329	353\\
70	44	107\\
107	44	68\\
135	102	70\\
153	102	135\\
70	107	135\\
135	107	163\\
135	187	153\\
135	163	187\\
129	100	66\\
215	186	242\\
215	244	188\\
258	204	234\\
230	204	258\\
501	464	444\\
464	391	444\\
307	281	358\\
154	191	212\\
212	181	154\\
212	191	248\\
237	181	212\\
248	264	212\\
212	264	237\\
209	181	237\\
209	238	183\\
209	183	151\\
151	181	209\\
323	264	292\\
323	292	339\\
339	375	323\\
323	375	350\\
298	238	261\\
261	326	298\\
261	209	237\\
238	209	261\\
262	238	298\\
262	299	239\\
183	238	210\\
210	262	239\\
238	262	210\\
531	538	506\\
506	538	477\\
526	538	578\\
477	538	526\\
526	492	457\\
457	477	526\\
433	492	462\\
462	406	433\\
548	526	578\\
492	526	548\\
546	581	522\\
545	521	582\\
21	19	83\\
21	84	24\\
83	84	21\\
198	144	200\\
168	144	198\\
224	168	198\\
200	250	198\\
198	250	224\\
112	144	168\\
79	144	112\\
80	79	112\\
112	138	80\\
112	168	138\\
363	389	419\\
363	335	313\\
363	313	337\\
337	389	363\\
363	419	390\\
390	335	363\\
387	389	337\\
387	417	448\\
387	448	443\\
443	389	387\\
418	391	464\\
418	464	474\\
474	417	418\\
503	448	474\\
503	500	448\\
562	500	503\\
474	504	503\\
503	504	566\\
566	562	503\\
570	508	556\\
508	500	556\\
556	500	562\\
354	286	330\\
285	356	330\\
257	285	330\\
330	286	257\\
382	354	330\\
330	356	382\\
331	356	285\\
285	256	331\\
331	256	284\\
331	284	355\\
331	355	384\\
384	356	331\\
454	393	427\\
420	393	454\\
454	484	530\\
427	484	454\\
530	476	454\\
454	476	420\\
156	211	180\\
216	160	180\\
180	235	216\\
211	235	180\\
295	319	268\\
268	235	295\\
216	235	268\\
103	160	133\\
103	53	58\\
199	167	223\\
167	194	223\\
223	253	199\\
223	277	253\\
185	127	162\\
127	106	162\\
127	159	105\\
105	60	127\\
159	214	182\\
182	211	156\\
236	211	182\\
182	214	236\\
573	535	516\\
535	478	516\\
516	478	450\\
516	450	489\\
516	542	573\\
489	542	516\\
290	240	269\\
269	245	289\\
269	318	290\\
289	318	269\\
481	540	527\\
524	540	481\\
425	455	481\\
481	455	524\\
460	402	425\\
425	481	460\\
460	481	527\\
528	536	585\\
486	463	528\\
528	537	486\\
585	537	528\\
376	351	405\\
405	351	373\\
486	467	431\\
431	463	486\\
431	407	376\\
467	407	431\\
376	405	431\\
431	405	463\\
239	299	265\\
6	39	64\\
64	39	96\\
64	40	6\\
97	40	64\\
64	96	126\\
126	97	64\\
99	66	41\\
99	129	66\\
130	61	110\\
110	166	130\\
154	95	130\\
130	95	61\\
130	191	154\\
130	166	191\\
234	208	260\\
134	68	104\\
134	192	163\\
134	107	68\\
163	107	134\\
187	163	219\\
163	192	219\\
301	244	267\\
267	215	242\\
244	215	267\\
131	100	158\\
100	129	158\\
158	129	186\\
188	131	158\\
158	215	188\\
186	215	158\\
228	202	255\\
255	202	230\\
357	329	383\\
281	254	333\\
333	358	281\\
515	550	493\\
515	572	550\\
485	541	515\\
541	572	515\\
553	565	496\\
413	472	438\\
264	323	293\\
326	261	293\\
350	326	293\\
293	323	350\\
237	264	293\\
293	261	237\\
155	97	126\\
155	126	183\\
183	210	155\\
477	421	447\\
447	506	477\\
447	421	392\\
298	326	349\\
350	406	378\\
404	349	378\\
378	326	350\\
378	349	326\\
525	462	492\\
492	548	525\\
525	548	579\\
525	579	549\\
406	462	436\\
436	378	406\\
404	378	436\\
519	544	576\\
519	480	453\\
543	519	576\\
480	519	543\\
430	488	458\\
458	488	521\\
521	488	547\\
547	582	521\\
522	581	547\\
547	488	522\\
446	444	415\\
415	444	391\\
391	360	415\\
156	180	120\\
120	180	160\\
120	101	156\\
58	101	120\\
120	103	58\\
160	103	120\\
249	194	216\\
216	268	249\\
249	223	194\\
277	223	249\\
310	277	296\\
296	268	319\\
296	338	310\\
296	319	338\\
277	249	296\\
296	249	268\\
1	53	57\\
53	103	57\\
57	103	133\\
57	133	111\\
57	54	1\\
57	111	54\\
185	162	217\\
217	240	185\\
245	269	217\\
217	269	240\\
132	106	63\\
132	162	106\\
63	108	132\\
132	108	164\\
51	2	60\\
60	105	51\\
51	59	3\\
51	105	59\\
124	182	156\\
159	182	124\\
156	101	124\\
101	59	124\\
124	105	159\\
59	105	124\\
482	460	527\\
482	528	463\\
527	536	482\\
536	528	482\\
428	405	373\\
463	405	428\\
373	402	428\\
402	460	428\\
428	482	463\\
460	482	428\\
7	40	65\\
65	40	97\\
41	7	65\\
65	99	41\\
327	379	353\\
346	379	327\\
304	258	234\\
234	260	304\\
260	327	304\\
329	258	304\\
304	353	329\\
304	327	353\\
343	316	301\\
369	316	343\\
343	399	369\\
372	399	343\\
246	219	192\\
104	131	161\\
161	134	104\\
161	131	188\\
192	134	161\\
219	246	270\\
348	374	322\\
322	299	348\\
322	265	299\\
306	254	228\\
228	255	306\\
306	255	332\\
306	333	254\\
332	255	305\\
329	357	305\\
305	357	332\\
305	258	329\\
230	258	305\\
305	255	230\\
332	357	385\\
358	333	386\\
413	438	386\\
554	564	505\\
505	564	499\\
446	505	499\\
499	560	501\\
499	564	560\\
501	444	499\\
499	444	446\\
493	550	512\\
550	569	512\\
512	569	553\\
553	496	512\\
513	496	565\\
472	496	513\\
513	565	559\\
465	505	446\\
184	210	239\\
184	155	210\\
522	488	459\\
459	488	430\\
298	349	325\\
348	299	325\\
325	262	298\\
299	262	325\\
461	432	404\\
404	436	461\\
462	525	491\\
491	436	462\\
491	461	436\\
491	525	549\\
480	543	517\\
543	574	517\\
517	541	485\\
517	574	541\\
575	520	545\\
544	520	575\\
544	519	483\\
483	520	544\\
456	520	483\\
483	519	453\\
487	520	456\\
487	458	521\\
487	521	545\\
545	520	487\\
456	399	429\\
429	487	456\\
458	487	429\\
429	399	372\\
453	395	426\\
426	399	456\\
426	395	369\\
369	399	426\\
426	483	453\\
456	483	426\\
190	217	162\\
162	132	190\\
221	245	190\\
245	217	190\\
190	164	221\\
190	132	164\\
372	343	320\\
301	267	320\\
320	343	301\\
218	246	192\\
188	244	218\\
218	161	188\\
192	161	218\\
271	244	301\\
301	316	271\\
271	218	244\\
246	218	271\\
400	379	346\\
346	368	400\\
400	434	379\\
485	515	468\\
468	434	485\\
493	440	468\\
468	515	493\\
219	270	241\\
241	260	208\\
241	208	187\\
187	219	241\\
303	327	260\\
260	241	303\\
303	241	270\\
346	327	303\\
341	316	369\\
369	395	341\\
395	368	341\\
470	512	496\\
470	440	493\\
493	512	470\\
412	357	383\\
412	385	357\\
383	440	412\\
440	470	412\\
413	386	359\\
359	386	333\\
359	385	413\\
332	385	359\\
359	306	332\\
333	306	359\\
505	465	498\\
498	513	559\\
498	465	438\\
559	554	498\\
498	554	505\\
498	438	472\\
472	513	498\\
446	415	414\\
414	465	446\\
358	386	414\\
414	386	438\\
438	465	414\\
213	184	239\\
242	186	213\\
213	265	242\\
239	265	213\\
186	129	157\\
157	213	186\\
184	213	157\\
129	99	157\\
432	459	403\\
403	374	348\\
430	374	403\\
403	459	430\\
432	461	490\\
522	459	490\\
490	459	432\\
490	546	522\\
401	429	372\\
458	429	401\\
401	374	430\\
430	458	401\\
372	320	345\\
345	322	374\\
345	401	372\\
374	401	345\\
300	320	267\\
265	322	300\\
322	345	300\\
300	345	320\\
242	265	300\\
300	267	242\\
302	271	316\\
316	341	302\\
302	270	246\\
246	271	302\\
434	400	452\\
485	434	452\\
452	517	485\\
480	517	452\\
424	368	395\\
424	400	368\\
424	452	400\\
424	395	453\\
453	480	424\\
480	452	424\\
409	440	383\\
409	468	440\\
383	353	409\\
353	379	409\\
379	434	409\\
434	468	409\\
413	385	442\\
442	472	413\\
385	412	442\\
442	412	470\\
442	496	472\\
442	470	496\\
361	414	415\\
361	415	360\\
307	358	361\\
358	414	361\\
361	309	307\\
361	360	309\\
155	184	128\\
184	157	128\\
97	155	128\\
128	65	97\\
99	65	128\\
128	157	99\\
404	432	377\\
432	403	377\\
377	349	404\\
377	403	348\\
348	325	377\\
377	325	349\\
461	491	523\\
523	490	461\\
549	580	523\\
523	491	549\\
580	546	523\\
546	490	523\\
317	303	270\\
270	302	317\\
346	303	317\\
317	302	341\\
317	368	346\\
317	341	368\\
}]
table[row sep=crcr, point meta=\thisrow{c}] {%
x	y	c\\
-0.500000000128793	2.04132776030805	0.000341488067861453\\
-0.500000000129399	2.22594022862531	-0.000620050675743092\\
-0.500000000127528	1.67670471017953	-0.0128345549470672\\
-0.500000000128184	1.85827645522055	-0.00584307640363716\\
-0.500000000126959	-2.32836587503923	-0.00393789664431559\\
-0.500000000126798	-2.15429021569747	0.000701242226727051\\
-0.500000000126742	-1.98013660312688	-0.00111739680316086\\
-0.500000000126642	-1.80584377943372	-0.0081555940542213\\
-0.500000000126511	-1.63140394149421	-0.0137652630233192\\
-0.50000000012676	1.49673476014683	-0.0135891743054451\\
-0.500000000126301	-1.45680683940949	-0.0127290579775208\\
-0.500000000125886	-1.28214828875708	-0.00664630200327721\\
-0.500000000125567	1.31865105175289	-0.00802680655106485\\
-0.500000000124902	-1.10782894274147	-0.0022191923278412\\
-0.500000000122732	1.14349809629118	-0.00267299214615795\\
-0.500000000121571	-0.935562921503897	-0.00408394146814991\\
-0.500000000112775	0.972640455490986	-0.00315918485458487\\
-0.500000000108685	0.259948841239582	0.000906438921725707\\
-0.500000000106369	-0.764859165398379	-0.00993924179249527\\
-0.500000000101702	-0.105696421239095	0.00909273039215636\\
-0.500000000101827	2.40951262596426	-0.00692052924629349\\
-0.500000000095918	-0.00658705726587586	0.0110651717642655\\
-0.500000000095119	-0.587605305719356	-0.0130611622773321\\
-0.500000000094258	-0.299962104419686	-0.00163544210627119\\
-0.500000000092581	0.08786760124241	0.00969028405276069\\
-0.500000000092646	0.801710482078886	-0.00865667195310255\\
-0.500000000092004	-0.489933941111698	-0.0113538699978535\\
-0.500000000091642	-0.204058458673054	0.00432445992714087\\
-0.500000000092123	0.346423712827746	-0.00451780842064753\\
-0.500000000087129	0.527438563099096	-0.0123307668827669\\
-0.50000000008631	0.623782575167252	-0.013008951866782\\
-0.50000000008471	0.175328402783412	0.00593025287627094\\
-0.500000000077986	0.708468495911193	-0.0116155667860056\\
-0.50000000007594	-0.399556815712473	-0.00752144940933299\\
-0.500000000074551	-0.672844160676831	-0.0123974393799998\\
-0.500000000066336	0.440832290563093	-0.00950775495588148\\
-0.500000000063868	0.883880191094239	-0.00570526168999163\\
-0.50000000005714	-0.847686364895949	-0.00698488561442457\\
-0.50000000005297	-2.2412066830433	-0.00102993242444367\\
-0.500000000052982	-2.0670358235305	0.000700001991334318\\
-0.500000000052409	-1.8927977124053	-0.004348737164079\\
-0.500000000051509	-1.7184332666223	-0.0115952531753906\\
-0.500000000050339	-1.54386971781278	-0.0141560667510126\\
-0.500000000048844	-1.36910417309693	-0.00993321538103432\\
-0.500000000046973	-1.19429616884305	-0.00378008897087915\\
-0.500000000045237	1.05547448378431	-0.00208631582116856\\
-0.500000000044383	-1.01994276775877	-0.0023619150134021\\
-0.500000000041887	-2.41536381624981	-0.00712375396411937\\
-0.500000000041272	1.40704591348788	-0.0112620459456312\\
-0.500000000041174	1.58634453825269	-0.0142054480240097\\
-0.500000000040376	1.22964807366878	-0.00481866911333163\\
-0.500000000040685	1.76716117380626	-0.0097830014275175\\
-0.50000000004002	1.94939687378611	-0.00212950998836717\\
-0.500000000039018	2.13299282189266	0.000873676108004227\\
-0.500000000022272	2.31792243512375	-0.00355518785151534\\
-0.5	-2.5	-0.00957864000189117\\
-0.5	2.5	-0.00957864008212799\\
-0.41788211498184	2.22375482643563	0.00337700900145061\\
-0.417645622072295	2.04027275049857	0.00510042332678726\\
-0.417435516304811	1.85763211290724	-3.76593810187667e-05\\
-0.417213583981939	1.67619585598195	-0.00566756400204178\\
-0.41702170717101	-2.32809520091121	-0.000348643258797286\\
-0.416970143433059	-2.15372164063704	0.00499293700288731\\
-0.416958941515121	1.49585573202455	-0.00473057707888041\\
-0.416952882542606	-1.97942220090185	0.0040014736006278\\
-0.41691919514277	-1.80515064684664	-0.00195913626797907\\
-0.416875098602677	-1.63066064611983	-0.00618131292686272\\
-0.416807787776402	-1.45581131854325	-0.00343522724774769\\
-0.416679482936078	-1.28059292949691	0.00469391490039618\\
-0.416584399075444	1.31660303225338	0.00290617212326546\\
-0.416393210584702	-1.10505070414049	0.011548429918065\\
-0.415814713743076	1.13832060424822	0.010748236474396\\
-0.41569989302031	-0.927986872958574	0.012595436825958\\
-0.415569587147517	2.49999999965392	-0.00655139240515445\\
-0.415012712383491	-0.553416049361979	0.0133917795976932\\
-0.414244297834606	-0.742131259506346	0.0105798654479321\\
-0.41415319855354	0.957160511687912	0.0131231324063352\\
-0.413918250413298	0.580284284659652	0.0126562025995718\\
-0.41334739400258	0.769385760119911	0.0110085844753744\\
-0.411054858504877	0.264367099192073	0.0369508302145281\\
-0.411008565460334	0.382121328756386	0.0262288286040764\\
-0.410184888062253	-2.49999999957771	-0.00633701893664143\\
-0.40991330364959	-0.354183003407736	0.0291009541228196\\
-0.409887615585548	-0.0483932850186597	0.050528234925092\\
-0.408535281405233	0.0631687930276817	0.0507117095098719\\
-0.407706747730726	2.40254378767514	-0.00295747064591505\\
-0.406466150566922	-0.15352078048192	0.0474078423093692\\
-0.403474172060161	0.165561589300292	0.0477650125252104\\
-0.400937210488816	-0.252371712032808	0.0417256702859461\\
-0.394451049655436	-0.460012900270388	0.0249897344980453\\
-0.390624062681736	0.486722678319409	0.0241319037831401\\
-0.39058833089668	-0.648305549949726	0.016826237387175\\
-0.38955421213571	0.676325505226407	0.0165945565100287\\
-0.388485684977008	0.862651055341308	0.0172404203079846\\
-0.38783936226423	-0.834802646804944	0.0171075127984858\\
-0.385022095932561	-2.24067106234406	0.00455842570505384\\
-0.385018272740042	-2.06639919172859	0.0073268727449607\\
-0.3848336253217	-1.8921901229315	0.00358817110272932\\
-0.384712880279827	1.04673591448212	0.0178422168124866\\
-0.384679729620522	-1.71785020010335	-0.00197434652309522\\
-0.384523674753782	-1.54317065881665	-0.00243971966168592\\
-0.384453975118491	1.9484902454238	0.00536598079354906\\
-0.384425020933973	-1.01591796587273	0.0182822257166272\\
-0.384357987494246	2.13138360170553	0.00713471230013292\\
-0.384303046415459	-1.36804976770566	0.00430628162161915\\
-0.384248625401657	1.76658358580813	-0.000635001148398517\\
-0.384059826338971	1.58570243574464	-0.00298844945809953\\
-0.384036632240582	-1.19246082276286	0.0134433497145553\\
-0.383815315514838	1.40575261016041	0.00247069353616083\\
-0.383544551958538	1.22661663843641	0.0119048571043737\\
-0.383347901277452	-2.41406322431196	-0.00233629446506626\\
-0.381324444903984	2.31303596982753	0.00198360909879539\\
-0.337563874955654	0.314235503330101	0.0545072318313319\\
-0.330148842665759	0.0108784818729889	0.0767908475476742\\
-0.330117912546826	2.49999999968702	-0.00313788226446074\\
-0.32346096850888	-0.558270262956205	0.0346736657677717\\
-0.322127016477104	0.587395829182225	0.0332637509789666\\
-0.321146670930549	-0.743583746786828	0.0289223232896402\\
-0.320121218879085	0.771502867443507	0.0288521144348426\\
-0.319203962600906	-0.924571560906267	0.0286873780354194\\
-0.318974085801103	2.03911397383485	0.0110261343940044\\
-0.318867305164175	0.95355455931136	0.028568264662758\\
-0.318802549712898	-0.396184147249353	0.0494001203359254\\
-0.318792731855836	-0.10073969698136	0.0773771308530259\\
-0.318697337520707	1.85704795500923	0.00695786446863547\\
-0.318629077135811	-2.15317460205693	0.0103538271870772\\
-0.31848432075206	-1.97913828961342	0.0102449606192864\\
-0.318356883845464	1.67576776767783	0.00267187115517622\\
-0.318325116754033	-1.80496217150871	0.00538899272653127\\
-0.318197473952311	-1.63048403486105	0.00251515867710029\\
-0.318068864030357	-2.32668422922917	0.00432972390116023\\
-0.318037737913208	-1.4555364924245	0.00684316059073818\\
-0.318005430504603	1.49528960664296	0.0051989639315931\\
-0.317961329316473	2.22104281309248	0.0085797159562589\\
-0.31778892857397	-1.27999954457478	0.0167777938452688\\
-0.317684910695158	-1.1034898559057	0.0256392637367882\\
-0.317549420326977	1.31543458639142	0.0146536426810164\\
-0.317500081566481	1.1352991247793	0.0244352795756768\\
-0.313448198549387	0.416229550725239	0.0482350959906182\\
-0.312488924162441	0.121837741368272	0.077703535759938\\
-0.311351186333611	-2.49999999955931	-0.00243383151780861\\
-0.310234820477491	-0.30275199020269	0.0614858144329823\\
-0.30781238156304	2.40310114769002	0.00132959059138576\\
-0.305134222161207	-0.195956274297042	0.0737843303565716\\
-0.302933188932858	0.218328135783773	0.0720457571407543\\
-0.280166063433939	-0.654473136019285	0.0358393708954164\\
-0.277989566101989	0.681884719365986	0.0352268687508794\\
-0.276068055649726	-0.835193323204116	0.0336114453225353\\
-0.275923084460394	0.863251533455751	0.0335440056643389\\
-0.274923607784589	-0.476073412353518	0.0472941242950939\\
-0.27431229353037	0.50511137265576	0.0448546860479746\\
-0.2730561454736	-2.06597310854146	0.013356754896328\\
-0.273045221868597	1.04413768513554	0.0317382740458296\\
-0.272908842671294	-1.0138788774259	0.0324299705284683\\
-0.272872484679137	-2.23959182632045	0.00985226242382353\\
-0.272818241413257	-1.89199656047714	0.0105419461140272\\
-0.272670028900443	1.94761583654341	0.0119655693943554\\
-0.27261639472014	-1.71773397678369	0.00611154839734561\\
-0.272430182691645	-1.5430251356466	0.00696707514899275\\
-0.272388660234676	1.7661048617755	0.00708218778158869\\
-0.272289192609185	2.12943959199927	0.0128832095538533\\
-0.272177533936117	-1.36772092787782	0.015177518754105\\
-0.27209897484684	1.58526625657322	0.00606058792124236\\
-0.271993989754244	-1.19156717323446	0.0258877594402212\\
-0.271777947648051	1.40502139171703	0.0130106579899605\\
-0.27167539932296	1.22489750399079	0.0240433053675964\\
-0.27088891961054	-2.41270535137311	0.00225990215367745\\
-0.268942682918708	2.31136620335749	0.00697360112916599\\
-0.249777399006616	0.327428632301962	0.0649321657249478\\
-0.246199143510991	-0.0434278908752602	0.0868667254012758\\
-0.242752242798228	0.0597607615946108	0.0869339949010077\\
-0.239395457403525	2.4999999996722	-0.000156881402935628\\
-0.226167208257579	-0.256065767617996	0.0738294942764281\\
-0.219654614557901	-0.375528897607227	0.0589842653163643\\
-0.219620507517468	-0.571159526241755	0.0420062654335022\\
-0.218207133596319	-0.746982214822454	0.0366607778215178\\
-0.216871147902582	0.773918661065838	0.0364555301683916\\
-0.216791013943207	0.597153694509699	0.0406104119662805\\
-0.215127359077835	-0.924579680473896	0.036099176916446\\
-0.21503838299676	0.953694643001166	0.0359063458531754\\
-0.21421514752066	2.03790076332547	0.0153065240064805\\
-0.214122111622725	-2.15244906801931	0.014350639204837\\
-0.214110940554071	1.85647861026013	0.0117410718897987\\
-0.214046041795409	-1.97887308906824	0.014666555136319\\
-0.213842566411091	-1.80487170686528	0.0103361291968366\\
-0.213776715861717	1.67542408553137	0.00806415075251127\\
-0.213687745618063	-1.63042436388134	0.00805971239726828\\
-0.213554806345005	-1.10248072826192	0.0326805841104462\\
-0.213510483820773	-1.45538799952159	0.0129888072897943\\
-0.213501946707498	1.13403000819466	0.0314172485696222\\
-0.213439281466423	1.49486826117829	0.0112213344362627\\
-0.21331418292525	-2.32563551911675	0.00793475590690125\\
-0.213310550882311	-1.2795482964621	0.0234442643594333\\
-0.213146915622256	1.31456145062978	0.0212335991847668\\
-0.212962425117144	2.21964002130615	0.0124415269607327\\
-0.208818154609576	-2.49999999954863	0.000533715079317922\\
-0.208657680297502	-0.137702478064195	0.0851764523668679\\
-0.208286673038878	0.419999214178588	0.053550132901237\\
-0.20620080286975	0.241476252424373	0.0746823373770254\\
-0.205532698583973	2.40330179602454	0.00443926046881978\\
-0.199360963103003	0.150848289222566	0.0839498313130923\\
-0.173265028684704	-0.480991496775203	0.0446776552586943\\
-0.168356553549101	-0.661705289550892	0.0356079278492703\\
-0.166018607446096	0.68682563617108	0.0349697729884248\\
-0.16538322325687	-0.836157898377143	0.0346870510693741\\
-0.165331403936399	0.864331237523037	0.0348242255863715\\
-0.163415103155835	0.511238362257546	0.0412510548247043\\
-0.163344558517944	1.04374690395256	0.0338225486005838\\
-0.16328015083799	-1.01348663687743	0.0343391203198005\\
-0.16325521830563	-2.06550383737885	0.0161375414700327\\
-0.163091834248517	-1.8918539896531	0.013450927544292\\
-0.163039448211965	1.94682164477094	0.0148082125681987\\
-0.163008750562248	-2.23872208713505	0.0125103072140762\\
-0.162919351232974	-1.71769485075286	0.00915705187270364\\
-0.162852105438069	1.76572153757401	0.0100704138755028\\
-0.162768345128281	-1.54296048698574	0.010083261907623\\
-0.162665392384179	2.12824338334097	0.0156033339747866\\
-0.162600433253431	1.584962565296	0.00915257477227634\\
-0.162585670649602	-1.36747442347954	0.0181860760870109\\
-0.162577682822946	-1.19095714580843	0.0285008624321204\\
-0.162407842371072	1.22402943297308	0.0267489925839006\\
-0.162367160489535	1.40449695492793	0.0160484012198066\\
-0.161585538057935	-2.41222602000894	0.0046526024588953\\
-0.160219917237363	2.31070354157829	0.00943525435477446\\
-0.148855106737316	0.327899234024683	0.0550056149987289\\
-0.145016465656958	2.49999999966171	0.0013023766250089\\
-0.143404875783038	-0.309817959978127	0.0558402829195825\\
-0.139777160906878	-0.207273600339185	0.06910361928248\\
-0.114377755858281	-0.575183743845226	0.0298970149022429\\
-0.113459656588949	-0.408871934675441	0.0385064781168367\\
-0.109480927881078	-0.749129450174653	0.02783805435602\\
-0.109091221640542	0.776375039050967	0.0281118890945122\\
-0.108342105817413	0.600058745650739	0.0280816340828119\\
-0.108143265765223	0.954030791000812	0.0303470742452986\\
-0.108084499924764	-0.924771172299884	0.0301158943935294\\
-0.107419557692027	2.03714631349168	0.0157930044001006\\
-0.107405053860496	1.85603289843674	0.011889465698877\\
-0.107405019646202	-2.15190190787273	0.0150142726117128\\
-0.107401595162553	-1.97862728490816	0.0150514702863739\\
-0.107271461380696	-1.80481698534424	0.010376469797851\\
-0.107212303835751	1.67518352259944	0.0077747112081265\\
-0.10718807226795	-1.10219918392812	0.0288490269329009\\
-0.10716387588133	-1.63040152441193	0.00763197504965237\\
-0.10715466863578	1.13367309447944	0.0279171329889103\\
-0.107050597615345	-1.45527746402443	0.0118532508825191\\
-0.107010986727095	1.49457675373655	0.0102750381985262\\
-0.106969759916143	-1.27921361765997	0.0212196242491348\\
-0.106894361497028	1.31406500790348	0.0192652201666745\\
-0.106880354500428	-2.32512537012707	0.00875418128461353\\
-0.106620850481248	2.218919482779	0.0131609323254802\\
-0.105886677173257	0.226468566491082	0.0559751960505216\\
-0.104710169322933	-2.49999999954299	0.00128145321246838\\
-0.104693577553929	0.423238170146931	0.0351047588993429\\
-0.102790382308323	2.40361024296636	0.00507050191435203\\
-0.059928084394661	-0.497074949023708	0.0187086868384544\\
-0.0566703238179262	-0.661808058601696	0.0165551633246978\\
-0.0552577606862261	0.688934035014045	0.0166279673664245\\
-0.0550709445467183	0.865325405268681	0.0212096072959391\\
-0.0548873198559098	-0.836772149226303	0.0203620999206677\\
-0.0544133718150923	1.04370480195096	0.0237860002131868\\
-0.0544126164536982	-1.01350035554521	0.0237652128799912\\
-0.0543412737376513	-2.06520465393553	0.0146140554297386\\
-0.0542880455376873	-1.89175579939783	0.0112431013300649\\
-0.054273697213948	1.946394960237	0.0128214727000873\\
-0.0542333249931837	-2.23831339288543	0.0115357226039054\\
-0.054220499497772	-1.71768293902027	0.00610948516622141\\
-0.0542097025970838	1.76549156795085	0.00726737379860323\\
-0.0541607024805681	-1.54292487736472	0.00593648534679227\\
-0.0541187215128513	2.12768869384547	0.0142889654525166\\
-0.0541129208505885	1.58479110902944	0.00529923369431916\\
-0.0541100765834874	-1.19072179035782	0.0207500595670905\\
-0.0541007662452783	-1.36731555477371	0.0125300638825624\\
-0.0540574863238427	1.22373255740342	0.0194436346422404\\
-0.0540341067605828	1.40422466059458	0.0107560521371401\\
-0.0540292901218352	0.329507715750734	0.0243381957962938\\
-0.0537287800682893	-2.41208456540782	0.0040273240136288\\
-0.0536803077245693	0.511876791342339	0.0164910240658769\\
-0.053242211821487	2.31053075719759	0.0085867825052617\\
-0.049099171261658	-0.245131130931619	0.0285920401092862\\
-0.0485577652529077	2.49999999965553	0.000604046213035426\\
-0.0469784477258105	-0.335300075839326	0.0211601939938227\\
-2.89044114042819e-09	-0.423788415245136	0.000256651685569047\\
-1.22844672004185e-09	0.250000000030766	0.00209722861785275\\
-4.59836312430295e-10	0.420101641885394	0.000297881174814627\\
-2.12390769901982e-10	0.601162931917671	0.000742117992833862\\
-9.29252334802566e-11	0.777139982213398	0.00676528948921698\\
-3.73701354583478e-11	0.954292819910273	0.0138403727262478\\
-1.57307483011904e-11	1.13356963713163	0.0152224028770782\\
-6.09257679029529e-12	1.31392716590624	0.009472684101985\\
-2.1506553482542e-12	1.49446835086784	0.00265534564635182\\
-7.08433312013312e-13	1.67509207320782	0.00179267927599316\\
9.42339956067073e-14	-2.4999999995413	-0.000527104346237072\\
2.12694445389516e-13	-2.32497954561041	0.00642052533449734\\
5.01750377357446e-13	-2.1517116710942	0.0119618134213091\\
-2.46542369852776e-13	1.85587231618647	0.00719108526656172\\
-9.84930886849256e-14	2.03689028023991	0.0121602003909644\\
-4.27307494943463e-14	2.21872090663795	0.0104177906243472\\
-1.96769683880049e-14	2.4037278237192	0.00301062066846045\\
1.29843254204065e-12	-1.97852567002465	0.0110974237913097\\
3.63973885753044e-12	-1.80479573657728	0.00534765630733973\\
1.10230474054118e-11	-1.63039648947411	0.00128390407208789\\
3.29307359159259e-11	-1.45522813705942	0.0038070659636575\\
9.38763074220805e-11	-1.27911406803773	0.0109234967891311\\
2.34340979954339e-10	-1.10210611503734	0.015565583085602\\
5.8581049837414e-10	-0.925115036130878	0.0129195072436853\\
1.10597096064646e-09	-0.748595468447535	0.0055330997073671\\
1.43338025788975e-09	-0.578158525561495	0.000343436051909714\\
0.0469782680430556	-0.335299967282443	-0.0183101690913949\\
0.0485577652528834	2.49999999965553	-0.00205493929895958\\
0.0490993646466123	-0.245131092290335	-0.0239581693433187\\
0.0532422118214296	2.3105307571976	0.00493947351133884\\
0.0536803071062406	0.51187679151818	-0.0174116997614765\\
0.0537287800685749	-2.4120845654078	0.000778941666967573\\
0.0540292885194522	0.329507716179327	-0.0213122095063242\\
0.0540341067533255	1.40422466059652	-0.000321573392488609\\
0.0540574863039154	1.22373255740794	0.00559292260374075\\
0.054100766356155	-1.3673155547497	0.000928074688262928\\
0.0541100768849957	-1.19072179028412	0.00630158112293368\\
0.0541129208481707	1.58479110903003	-0.00364304260576606\\
0.0541187215127252	2.1276886938455	0.00961687413636141\\
0.0541607025183175	-1.54292487735673	-0.00346544599289575\\
0.0542097025962799	1.765491567951	8.49631789280386e-06\\
0.0542204995101656	-1.71768293901809	-0.00156547833447085\\
0.054233324993816	-2.23831339288532	0.00746863856720813\\
0.0542736972136448	1.94639496023706	0.00695449270335292\\
0.0542880455419342	-1.89175579939708	0.00497678278709742\\
0.0543412737392281	-2.06520465393523	0.0095393473818734\\
0.0544126171953763	-1.01350035542365	0.00561894810437213\\
0.0544133717650819	1.04370480195906	0.00631468242918618\\
0.05488732154424	-0.836772148669323	-0.00246956615765356\\
0.0550709444284374	0.865325405289537	-0.000891496844639172\\
0.0552577604032131	0.688934035093133	-0.0110440966562702\\
0.0566703264989913	-0.661808057423233	-0.0127886075966435\\
0.0599280867654109	-0.497074944086553	-0.0197308255504577\\
0.102790382308286	2.40361024296636	-0.000891595201119199\\
0.104693576724443	0.423238170675021	-0.0357232909550793\\
0.104710169323115	-2.49999999954299	-0.00413064356600046\\
0.105886674511681	0.226468567735517	-0.0494511552278793\\
0.106620850481167	2.21891948277903	0.00541300563083164\\
0.106880354500838	-2.32512537012695	0.00196756251637378\\
0.106894361485563	1.31406500790961	-0.00386291565682453\\
0.106969760087627	-1.27921361757829	-0.00294469399960142\\
0.107010986723274	1.49457675373868	-0.00831360566191681\\
0.107050597675965	-1.45527746399677	-0.00763688762503802\\
0.107154668604772	1.13367309449214	-0.00111917797094555\\
0.10716387590137	-1.6304015244039	-0.00823200855588489\\
0.107188072733248	-1.1021991837178	-0.00136719903278884\\
0.1072123038345	1.67518352259999	-0.00729166271588398\\
0.107271461387571	-1.80481698534174	-0.00259187299342041\\
0.107401595165048	-1.97862728490721	0.00449975685343375\\
0.107405019647164	-2.15190190787236	0.00652120518072545\\
0.107405053860029	1.85603289843693	-0.000335365737315503\\
0.107419557691839	2.03714631349176	0.00597502018522129\\
0.108084500933424	-0.924771171833905	-0.00790329870626651\\
0.108143265695072	0.954030791025834	-0.00632110828251591\\
0.10834210541817	0.600058745896022	-0.0292520135550113\\
0.109091221478176	0.776375039128586	-0.0180197963835779\\
0.109480929914148	-0.749129448372259	-0.0200391889445223\\
0.113459588362857	-0.408871864751243	-0.0388134516516623\\
0.114377756658213	-0.575183738621951	-0.0320379892940525\\
0.139777255497351	-0.207273536291228	-0.0603826011619711\\
0.143404866314	-0.309817984390733	-0.0518222095404303\\
0.145016465656935	2.49999999966171	-0.00569069466323668\\
0.148855105317079	0.327899235158597	-0.0519800637052824\\
0.160219917237311	2.31070354157831	5.06129359204915e-05\\
0.161585538058199	-2.41222602000886	-0.00367260417542476\\
0.162367160483486	1.40449695493332	-0.0123154675804749\\
0.162407842352192	1.22402943298705	-0.00871435064011716\\
0.162577683092347	-1.19095714562079	-0.00848945771757434\\
0.162585670744533	-1.36747442340898	-0.0115140052936999\\
0.162600433251579	1.58496256529743	-0.0137521337254611\\
0.162665392384065	2.12824338334105	0.00363300255641667\\
0.162768345159762	-1.54296048696466	-0.0139913771073653\\
0.16285210543738	1.76572153757448	-0.00853358283123129\\
0.162919351243724	-1.71769485074636	-0.0105124754991224\\
0.163008750562828	-2.23872208713472	0.00211116020414745\\
0.163039448211692	1.94682164477113	-0.000227490975083057\\
0.163091834252392	-1.89185398965079	-0.00261384009189717\\
0.163255218307077	-2.06550383737796	0.00314401046673102\\
0.163280151532998	-1.01348663635733	-0.0120308431811816\\
0.163344558468447	1.04374690397992	-0.0108278534864943\\
0.163415102595805	0.511238362825488	-0.0461474484259336\\
0.165331403834043	0.864331237587028	-0.0215017129279737\\
0.165383224493415	-0.836157897193139	-0.0236660944353521\\
0.166018607219663	0.68682563636683	-0.0355274285028869\\
0.168356555112001	-0.66170528421293	-0.0377698806577134\\
0.173265000426989	-0.480991460604778	-0.0494608050898638\\
0.199360959169189	0.150848294479252	-0.0682677722712838\\
0.205532698583941	2.40330179602456	-0.0050738943580407\\
0.20620080181274	0.241476255528552	-0.0655372140879093\\
0.208286672337631	0.419999215282483	-0.0573370314309914\\
0.208657705542002	-0.137702439761739	-0.0679337935357323\\
0.208818154609738	-2.49999999954863	-0.00801610878184483\\
0.212962425117074	2.21964002130621	0.000292513861437726\\
0.213146915613541	1.31456145064155	-0.0149714399475596\\
0.213310551017951	-1.27954829631233	-0.0143817399231479\\
0.213314182925611	-2.32563551911651	-0.00267066004601862\\
0.213439281464111	1.49486826118143	-0.0178797530927616\\
0.213501946679242	1.13403000822262	-0.0140147646351779\\
0.213510483864388	-1.4553879994739	-0.0175169994441988\\
0.213554806707219	-1.10248072786451	-0.0146008494802959\\
0.213687745633352	-1.63042436386662	-0.016797811506155\\
0.213776715860809	1.67542408553237	-0.015545984943696\\
0.213842566416787	-1.80487170686021	-0.0100158091964191\\
0.214046041797566	-1.97887308906635	-0.00188365530076708\\
0.21411094055369	1.85647861026052	-0.00743068189018272\\
0.214122111623565	-2.15244906801858	0.00106910554565962\\
0.214215147520501	2.03790076332563	-7.5756137752197e-05\\
0.215038382939643	0.95369464305871	-0.0212342088940384\\
0.215127359912632	-0.924579679335042	-0.0231697312081603\\
0.216791013671571	0.597153694924929	-0.0487847362321022\\
0.216871147791634	0.773918661204496	-0.0352290128328081\\
0.218207133947086	-0.746982211886085	-0.037598777694309\\
0.219620497169853	-0.571159506875843	-0.0507031919298086\\
0.21965460780556	-0.375528902016949	-0.0603093722414854\\
0.226167210261811	-0.256065780309419	-0.0656114602133652\\
0.239395457403505	2.4999999996722	-0.00897657769669469\\
0.242752239192086	0.0597607756845456	-0.0625479087782524\\
0.246199148291985	-0.0434278644859403	-0.061619854171024\\
0.249777398172105	0.327428634535164	-0.0631805976790549\\
0.268942682918666	2.31136620335753	-0.00403101035189938\\
0.270888919610758	-2.41270535137298	-0.00741933885526081\\
0.271675399307466	1.22489750401411	-0.0172513728876088\\
0.271777947644918	1.40502139172304	-0.0200062267214285\\
0.271993989961177	-1.19156717293554	-0.0171732642564994\\
0.272098974845711	1.58526625657515	-0.0206345135898091\\
0.272177534000397	-1.36772092778298	-0.0193646516002339\\
0.272289192609096	2.1294395919994	-0.00106945880737103\\
0.27238866023418	1.76610486177625	-0.0146615777928371\\
0.272430182713006	-1.54302513561591	-0.0210514126623693\\
0.272616394728193	-1.71773397677309	-0.01685193045832\\
0.272670028900234	1.94761583654372	-0.00561173581744385\\
0.272818241416317	-1.89199656047325	-0.00824784020401648\\
0.272872484679607	-2.23959182631989	-0.00219823933513852\\
0.272908843172344	-1.01387887664174	-0.0214566431860044\\
0.273045221820345	1.04413768518904	-0.020122829196311\\
0.27305614547477	-2.06597310853997	-0.00179063123591253\\
0.274312293150473	0.505111373432563	-0.0564362045831231\\
0.274923598514644	-0.476073412377653	-0.0576518776947068\\
0.27592308437548	0.863251533573009	-0.0313458306847555\\
0.27606805642772	-0.835193320643223	-0.0335690919796926\\
0.27798956597077	0.681884719649732	-0.0458170048944249\\
0.280166058238826	-0.654473126929754	-0.0477925365259779\\
0.302933187602607	0.218328138320138	-0.0601820853117614\\
0.305134217489432	-0.195956272962946	-0.0596485216376574\\
0.307812381563018	2.40310114769004	-0.0078800018402757\\
0.310234821842534	-0.302751992639821	-0.0587905917817097\\
0.311351186333738	-2.49999999955931	-0.0106007174383343\\
0.31248892495888	0.121837746598754	-0.0568365634751724\\
0.313448198340556	0.416229552166742	-0.0567926414894814\\
0.317500081547656	1.13529912482526	-0.0182403249869161\\
0.317549420325147	1.31543458640237	-0.0193009152017105\\
0.317684910907779	-1.10348985534013	-0.0187823741161203\\
0.317788928639574	-1.27999954439456	-0.0186957450632034\\
0.317961329316422	2.22104281309258	-0.00279346123198964\\
0.318005430503821	1.49528960664633	-0.0220821185597718\\
0.318037737935816	-1.4555364923666	-0.0217411862638776\\
0.318068864030635	-2.3266842292288	-0.00553611590072312\\
0.31819747396156	-1.63048403484053	-0.0208642265381009\\
0.318325116757887	-1.80496217150121	-0.0138544031101783\\
0.318356883844966	1.67576776767915	-0.0195505630372359\\
0.318484320753629	-1.97913828961056	-0.00540455367457424\\
0.318629077136446	-2.15317460205584	-0.00209905274802346\\
0.318697337520458	1.85704795500978	-0.0111537877302723\\
0.318792742789745	-0.100739687218635	-0.0549730586435605\\
0.318802546116105	-0.396184148997793	-0.0564859559860519\\
0.318867305133305	0.953554559413175	-0.0249684424365814\\
0.31897408580099	2.03911397383509	-0.00345488902753175\\
0.319203962838591	-0.924571559407736	-0.0267754761020863\\
0.320121218829773	0.771502867658136	-0.0380050689716397\\
0.321146669435801	-0.743583741246022	-0.0400600719748177\\
0.322127016380066	0.587395829692996	-0.0500055537340292\\
0.323460966232821	-0.558270260420588	-0.0512586395841225\\
0.330117912546808	2.49999999968702	-0.0108469770623228\\
0.330148847570029	0.0108784913663177	-0.0508646615580058\\
0.337563873981136	0.314235505175242	-0.0539160291802602\\
0.38132444490396	2.31303596982759	-0.00545658688513461\\
0.383347901277587	-2.41406322431176	-0.00875801379889057\\
0.383544551953599	1.22661663845135	-0.0160831320164402\\
0.383815315514185	1.40575261016545	-0.0198230331550311\\
0.384036632339169	-1.19246082245654	-0.0157172615368651\\
0.384059826338499	1.58570243574681	-0.0211278062301128\\
0.384248625401406	1.76658358580909	-0.0156056492979846\\
0.384303046443168	-1.36804976760283	-0.0189561383024043\\
0.384357987494196	2.13138360170572	-0.0023576427167182\\
0.384425021216812	-1.01591796485094	-0.0182906146691551\\
0.384453975118376	1.94849024542423	-0.00678440576995863\\
0.384523674764389	-1.54317065877858	-0.0213765527621106\\
0.384679729624872	-1.7178502000888	-0.0176899396550377\\
0.384712880234183	1.04673591456216	-0.017241674291618\\
0.384833625323477	-1.89219012292588	-0.00938250511831126\\
0.385018272740742	-2.06639919172639	-0.00303824954386685\\
0.385022095932845	-2.24067106234323	-0.00348647294894825\\
0.387839361784046	-0.834802644091847	-0.0276825669558984\\
0.388485684909086	0.862651055548971	-0.0258472911722163\\
0.389554212098792	0.676325505614704	-0.0369513137045002\\
0.390588329269749	-0.648305547774063	-0.0381152108607707\\
0.390624062626881	0.48672267928331	-0.0423484696506804\\
0.394451046557948	-0.460012899945242	-0.0415584161820143\\
0.400937208897334	-0.25237171173049	-0.0358836646207663\\
0.403474172701886	0.165561593452921	-0.0321914359804438\\
0.406466149988173	-0.153520781657327	-0.0307403853446872\\
0.407706747730717	2.40254378767517	-0.00823854907419814\\
0.408535283777139	0.0631687981352465	-0.0276242682737854\\
0.409887619754536	-0.0483932812400991	-0.0268923120546427\\
0.409913303484731	-0.354183004396527	-0.03599103633518\\
0.410184888062328	-2.49999999957771	-0.0109660224640301\\
0.411008565426439	0.382121330450743	-0.0363169105297642\\
0.411054857549356	0.26436710229521	-0.0329242790717626\\
0.413347394018385	0.769385760427828	-0.0280610635467166\\
0.413918250481403	0.580284285302273	-0.035858077698348\\
0.414153198591515	0.957160511847733	-0.0176689063738866\\
0.41424429737542	-0.742131257564913	-0.0294120715523522\\
0.415012712142481	-0.553416048396565	-0.0360995784604912\\
0.415569587147504	2.49999999965392	-0.0109191921961684\\
0.415699892895582	-0.927986871334849	-0.0188520724499828\\
0.415814713755067	1.13832060426986	-0.0131456536427507\\
0.416393210547037	-1.10505070363065	-0.0132776349259569\\
0.416584399077704	1.31660303225937	-0.015820336941465\\
0.416679482937056	-1.28059292933045	-0.0149055009977542\\
0.416807787781404	-1.45581131847935	-0.0192055336965226\\
0.416875098605939	-1.6306606460946	-0.0192818657741574\\
0.416919195144459	-1.8051506468366	-0.0129687249052925\\
0.416952882543398	-1.97942220089786	-0.00498104584243513\\
0.416958941515322	1.49585573202764	-0.0197836399983668\\
0.416970143433413	-2.15372164063547	-0.00196666975920541\\
0.417021707171171	-2.32809520091067	-0.00563629353982296\\
0.417213583981819	1.67619585598345	-0.0181511135078372\\
0.417435516304707	1.85763211290794	-0.0103912628497185\\
0.417645622072239	2.04027275049888	-0.00310563556612337\\
0.417882114981814	2.22375482643576	-0.0027837903596346\\
0.5	-2.5	-0.00935478981058539\\
0.5	2.5	-0.00935478981075635\\
0.500000000022272	2.31792243512384	-0.00331664148048012\\
0.500000000039018	2.13299282189291	0.000577021340107485\\
0.500000000040376	1.22964807366409	-0.00512201037777104\\
0.500000000040685	1.76716117380743	-0.0106051055774498\\
0.50000000004002	1.94939687378669	-0.00295750333567726\\
0.500000000041887	-2.41536381624947	-0.00681258791203009\\
0.500000000041272	1.40704591348968	-0.0113183849659558\\
0.500000000041174	1.58634453825465	-0.0145746336946807\\
0.500000000044383	-1.01994276748173	-0.00340540241587717\\
0.500000000045237	1.05547448374141	-0.0030073150466023\\
0.500000000046973	-1.19429616865633	-0.00419473197861628\\
0.500000000048844	-1.36910417300242	-0.009991347151442\\
0.500000000050339	-1.5438697177689	-0.0144152452004774\\
0.500000000052409	-1.89279771239695	-0.00524225488662326\\
0.500000000051509	-1.71843326660284	-0.0123199332325621\\
0.50000000005297	-2.24120668304196	-0.000968700567317935\\
0.500000000052982	-2.06703582352703	0.000175722840600972\\
0.50000000005714	-0.847686364933346	-0.00836879402234479\\
0.500000000063868	0.883880191062053	-0.00706273903129243\\
0.500000000066336	0.440832290546694	-0.0100767459998335\\
0.500000000074551	-0.672844160459472	-0.0135698941827546\\
0.50000000007594	-0.399556816266833	-0.00803078736636788\\
0.500000000077986	0.708468495963261	-0.0128691916399887\\
0.50000000008471	0.175328401085264	0.00533028027632462\\
0.50000000008631	0.623782575259921	-0.0140501829637381\\
0.500000000087129	0.527438563161906	-0.0130962922616203\\
0.500000000092004	-0.489933940871566	-0.0120241259394446\\
0.500000000091642	-0.204058459446529	0.00376500125221397\\
0.500000000092123	0.346423712309252	-0.00498800074069291\\
0.500000000092581	0.0878676010860515	0.00897511342891711\\
0.500000000092646	0.801710482062845	-0.0100362040536853\\
0.500000000094258	-0.299962104759339	-0.00210632378750317\\
0.500000000095119	-0.587605305618807	-0.0139978997339317\\
0.500000000095918	-0.00658705681172713	0.0103031499364583\\
0.500000000101702	-0.105696422188888	0.00839735553982118\\
0.500000000101827	2.40951262596429	-0.00660837515167209\\
0.500000000106369	-0.764859165573217	-0.0112862438000794\\
0.500000000108685	0.259948839294586	0.000410773545050146\\
0.500000000112775	0.972640455418504	-0.00434504956621844\\
0.500000000121571	-0.935562921826308	-0.00535871605083258\\
0.500000000122732	1.14349809625898	-0.00326744686331095\\
0.500000000124902	-1.10782894261958	-0.0029468043409123\\
0.500000000126301	-1.45680683934563	-0.0128246856400245\\
0.500000000125886	-1.28214828863911	-0.00681624573379429\\
0.500000000125567	1.31865105175039	-0.00813190249990688\\
0.500000000126959	-2.32836587503839	-0.00368273670926697\\
0.500000000126798	-2.15429021569507	0.000479720519848558\\
0.500000000126742	-1.98013660312098	-0.00188538174656096\\
0.500000000126642	-1.80584377941999	-0.00903000932510931\\
0.500000000126511	-1.63140394146368	-0.0142604639831389\\
0.50000000012676	1.49673476014859	-0.0137468423298151\\
0.500000000127528	1.67670471018111	-0.0134549741963137\\
0.500000000128184	1.85827645522143	-0.00674626078144895\\
0.500000000128793	2.04132776030847	-0.000264162511985386\\
0.500000000129399	2.22594022862548	-0.000603819723793471\\
};
%\addlegendentry{data3}

\end{axis}
%\end{tikzpicture}%

\node[align=center,anchor=north west,text opacity=1,rounded corners,fill=white,opacity=0,text opacity=1]
at (2er.north east) {(o)};
